Learning Towards the Largest Margins

One of the main challenges for feature representation in deep learning-based classification is the design of appropriate loss functions that exhibit strong discriminative power. The classical softmax loss does not explicitly encourage discriminative learning of features. A popular direction of research is to incorporate margins in well-established losses in order to enforce extra intra-class compactness and inter-class separability, which, however, were developed through heuristic means, as opposed to rigorous mathematical principles. In this work, we attempt to address this limitation by formulating the principled optimization objective as learning towards the largest margins. Specifically, we firstly define the class margin as the measure of inter-class separability, and the sample margin as the measure of intra-class compactness. Accordingly, to encourage discriminative representation of features, the loss function should promote the largest possible margins for both classes and samples. Furthermore, we derive a generalized margin softmax loss to draw general conclusions for the existing margin-based losses. Not only does this principled framework offer new perspectives to understand and interpret existing margin-based losses, but it also provides new insights that can guide the design of new tools, including sample margin regularization and largest margin softmax loss for the class-balanced case, and zero-centroid regularization for the class-imbalanced case. Experimental results demonstrate the effectiveness of our strategy on a variety of tasks, including visual classification, imbalanced classification, person re-identification, and face verification.

==> figures/hists/arcface-10.tex <==
\begin{figure}[tbp]
    \centering
    \subfigure[$\mu=0$]{
    \label{cifar10-hist-arcface-10-sim}
    \includegraphics[width=0.8in]{figures/hists/cifar10/cifar10_ArcFace_10_0.0_sim.png}
    }
    \subfigure[$\mu=0.5$]{
    \label{cifar10-hist-arcface-10-0.5-sim}
    \includegraphics[width=0.8in]{figures/hists/cifar10/cifar10_ArcFace_10_0.5_sim.png}
    }
    \subfigure[$\mu=1$]{
    \label{cifar10-hist-arcface-10-1-sim}
    \includegraphics[width=0.8in]{figures/hists/cifar10/cifar10_ArcFace_10_0.5_sim.png}
    }
    \subfigure[$\mu=0$]{
    \label{cifar10-hist-arcface-10-sm}
    \includegraphics[width=0.8in]{figures/hists/cifar10/cifar10_ArcFace_10_0.0_sm.png}
    }
    \subfigure[$\mu=0.5$]{
    \label{cifar10-hist-arcface-10-0.5-sm}
    \includegraphics[width=0.8in]{figures/hists/cifar10/cifar10_ArcFace_10_0.5_sm.png}
    }
    \subfigure[$\mu=1$]{
    \label{cifar10-hist-arcface-10-1-sm}
    \includegraphics[width=0.8in]{figures/hists/cifar10/cifar10_ArcFace_10_0.5_sm.png}
    }
    \subfigure[$\mu=0$]{
    \label{cifar100-hist-arcface-10-sim}
    \includegraphics[width=0.8in]{figures/hists/cifar100/cifar100_ArcFace_10_0.0_sim.png}
    }
    \subfigure[$\mu=0.5$]{
    \label{cifar100-hist-arcface-10-0.5-sim}
    \includegraphics[width=0.8in]{figures/hists/cifar100/cifar100_ArcFace_10_0.5_sim.png}
    }
    \subfigure[$\mu=1$]{
    \label{cifar100-hist-arcface-10-1-sim}
    \includegraphics[width=0.8in]{figures/hists/cifar100/cifar100_ArcFace_10_0.5_sim.png}
    }
    \subfigure[$\mu=0$]{
    \label{cifar100-hist-arcface-10-sm}
    \includegraphics[width=0.8in]{figures/hists/cifar100/cifar100_ArcFace_10_0.0_sm.png}
    }
    \subfigure[$\mu=0.5$]{
    \label{cifar100-hist-arcface-10-0.5-sm}
    \includegraphics[width=0.8in]{figures/hists/cifar100/cifar100_ArcFace_10_0.5_sm.png}
    }
    \subfigure[$\mu=1$]{
    \label{cifar100-hist-arcface-10-1-sm}
    \includegraphics[width=0.8in]{figures/hists/cifar100/cifar100_ArcFace_10_0.5_sm.png}
    }
    \caption{Histogram of similarities and sample margins for ArcFace ($s=10$) with/without sample margin regularization $R_{\text{sm}}$ on CIFAR-10 and CIFAR-100. (a-c) and (g-i) denote the cosine similarities on CIFAR-10 and CIFAR-100, respectively. (d-f) and (j-l) denote the sample margins on CIFAR-10 and CIFAR-100, respectively.
    }
    \label{fig:arcface-10-cifar10-hist}
    \vskip-10pt
\end{figure}

==> figures/hists/arcface-5.tex <==
\begin{figure}[tbp]
    \centering
    \subfigure[$\mu=0$]{
    \label{cifar10-hist-arcface-5-sim}
    \includegraphics[width=0.8in]{figures/hists/cifar10/cifar10_ArcFace_5_0.0_sim.png}
    }
    \subfigure[$\mu=0.5$]{
    \label{cifar10-hist-arcface-5-0.5-sim}
    \includegraphics[width=0.8in]{figures/hists/cifar10/cifar10_ArcFace_5_0.5_sim.png}
    }
    \subfigure[$\mu=1$]{
    \label{cifar10-hist-arcface-5-1-sim}
    \includegraphics[width=0.8in]{figures/hists/cifar10/cifar10_ArcFace_5_0.5_sim.png}
    }
    \subfigure[$\mu=0$]{
    \label{cifar10-hist-arcface-5-sm}
    \includegraphics[width=0.8in]{figures/hists/cifar10/cifar10_ArcFace_5_0.0_sm.png}
    }
    \subfigure[$\mu=0.5$]{
    \label{cifar10-hist-arcface-5-0.5-sm}
    \includegraphics[width=0.8in]{figures/hists/cifar10/cifar10_ArcFace_5_0.5_sm.png}
    }
    \subfigure[$\mu=1$]{
    \label{cifar10-hist-arcface-5-1-sm}
    \includegraphics[width=0.8in]{figures/hists/cifar10/cifar10_ArcFace_5_0.5_sm.png}
    }
    \subfigure[$\mu=0$]{
    \label{cifar100-hist-arcface-5-sim}
    \includegraphics[width=0.8in]{figures/hists/cifar100/cifar100_ArcFace_5_0.0_sim.png}
    }
    \subfigure[$\mu=0.5$]{
    \label{cifar100-hist-arcface-5-0.5-sim}
    \includegraphics[width=0.8in]{figures/hists/cifar100/cifar100_ArcFace_5_0.5_sim.png}
    }
    \subfigure[$\mu=1$]{
    \label{cifar100-hist-arcface-5-1-sim}
    \includegraphics[width=0.8in]{figures/hists/cifar100/cifar100_ArcFace_5_0.5_sim.png}
    }
    \subfigure[$\mu=0$]{
    \label{cifar100-hist-arcface-5-sm}
    \includegraphics[width=0.8in]{figures/hists/cifar100/cifar100_ArcFace_5_0.0_sm.png}
    }
    \subfigure[$\mu=0.5$]{
    \label{cifar100-hist-arcface-5-0.5-sm}
    \includegraphics[width=0.8in]{figures/hists/cifar100/cifar100_ArcFace_5_0.5_sm.png}
    }
    \subfigure[$\mu=1$]{
    \label{cifar100-hist-arcface-5-1-sm}
    \includegraphics[width=0.8in]{figures/hists/cifar100/cifar100_ArcFace_5_0.5_sm.png}
    }
    \caption{Histogram of similarities and sample margins for ArcFace ($s=5$) with/without sample margin regularization $R_{\text{sm}}$ on CIFAR-10 and CIFAR-100. (a-c) and (g-i) denote the cosine similarities on CIFAR-10 and CIFAR-100, respectively. (d-f) and (j-l) denote the sample margins on CIFAR-10 and CIFAR-100, respectively.
    }
    \label{fig:arcface-5-cifar10-hist}
    \vskip-10pt
\end{figure}

==> figures/hists/cifar100-cosface-64.tex <==
\begin{figure}[htbp]
    \centering
    \subfigure[CosFace ($s=64$)]{
    \label{cifar100-hist-cosface-64-sim}
    \includegraphics[width=1.7in]{figures/hists/cifar100/cifar100_CosFace_64_0.0_sim.png}
    }
    \subfigure[CosFace ($s=64$) + $0.5R_{\text{sm}}$]{
    \label{cifar100-hist-cosface-64-0.5-sim}
    \includegraphics[width=1.7in]{figures/hists/cifar100/cifar100_CosFace_64_0.5_sim.png}
    }
    \subfigure[CosFace ($s=64$) + $R_{\text{sm}}$]{
    \label{cifar100-hist-cosface-64-1-sim}
    \includegraphics[width=1.7in]{figures/hists/cifar100/cifar100_CosFace_64_0.5_sim.png}
    }
    \subfigure[CosFace ($s=64$)]{
    \label{cifar100-hist-cosface-64-sm}
    \includegraphics[width=1.7in]{figures/hists/cifar100/cifar100_CosFace_64_0.0_sm.png}
    }
    \subfigure[CosFace ($s=64$) + $0.5R_{\text{sm}}$]{
    \label{cifar100-hist-cosface-64-0.5-sm}
    \includegraphics[width=1.7in]{figures/hists/cifar100/cifar100_CosFace_64_0.5_sm.png}
    }
    \subfigure[CosFace ($s=64$) + $R_{\text{sm}}$]{
    \label{cifar100-hist-cosface-64-1-sm}
    \includegraphics[width=1.7in]{figures/hists/cifar100/cifar100_CosFace_64_0.5_sm.png}
    }
    \caption{Histogram of similarities and sample margins for CosFace with/without sample margin regularization $R_{\text{sm}}$ on CIFAR-100. (a-c) denote the cosine similarities between samples and their corresponding prototypes, and (d-f) denote the sample margins.
    }
    \label{fig:cosface-64-cifar100-hist}
    \vskip-10pt
\end{figure}

==> figures/hists/cosface-10.tex <==
\begin{figure}[tbp]
    \centering
    \subfigure[$\mu=0$]{
    \label{cifar10-hist-cosface-10-sim}
    \includegraphics[width=0.8in]{figures/hists/cifar10/cifar10_CosFace_10_0.0_sim.png}
    }
    \subfigure[$\mu=0.5$]{
    \label{cifar10-hist-cosface-10-0.5-sim}
    \includegraphics[width=0.8in]{figures/hists/cifar10/cifar10_CosFace_10_0.5_sim.png}
    }
    \subfigure[$\mu=1$]{
    \label{cifar10-hist-cosface-10-1-sim}
    \includegraphics[width=0.8in]{figures/hists/cifar10/cifar10_CosFace_10_0.5_sim.png}
    }
    \subfigure[$\mu=0$]{
    \label{cifar10-hist-cosface-10-sm}
    \includegraphics[width=0.8in]{figures/hists/cifar10/cifar10_CosFace_10_0.0_sm.png}
    }
    \subfigure[$\mu=0.5$]{
    \label{cifar10-hist-cosface-10-0.5-sm}
    \includegraphics[width=0.8in]{figures/hists/cifar10/cifar10_CosFace_10_0.5_sm.png}
    }
    \subfigure[$\mu=1$]{
    \label{cifar10-hist-cosface-10-1-sm}
    \includegraphics[width=0.8in]{figures/hists/cifar10/cifar10_CosFace_10_0.5_sm.png}
    }
    \subfigure[$\mu=0$]{
    \label{cifar100-hist-cosface-10-sim}
    \includegraphics[width=0.8in]{figures/hists/cifar100/cifar100_CosFace_10_0.0_sim.png}
    }
    \subfigure[$\mu=0.5$]{
    \label{cifar100-hist-cosface-10-0.5-sim}
    \includegraphics[width=0.8in]{figures/hists/cifar100/cifar100_CosFace_10_0.5_sim.png}
    }
    \subfigure[$\mu=1$]{
    \label{cifar100-hist-cosface-10-1-sim}
    \includegraphics[width=0.8in]{figures/hists/cifar100/cifar100_CosFace_10_0.5_sim.png}
    }
    \subfigure[$\mu=0$]{
    \label{cifar100-hist-cosface-10-sm}
    \includegraphics[width=0.8in]{figures/hists/cifar100/cifar100_CosFace_10_0.0_sm.png}
    }
    \subfigure[$\mu=0.5$]{
    \label{cifar100-hist-cosface-10-0.5-sm}
    \includegraphics[width=0.8in]{figures/hists/cifar100/cifar100_CosFace_10_0.5_sm.png}
    }
    \subfigure[$\mu=1$]{
    \label{cifar100-hist-cosface-10-1-sm}
    \includegraphics[width=0.8in]{figures/hists/cifar100/cifar100_CosFace_10_0.5_sm.png}
    }
    \caption{Histogram of similarities and sample margins for CosFace ($s=10$) with/without sample margin regularization $R_{\text{sm}}$ on CIFAR-10 and CIFAR-100. (a-c) and (g-i) denote the cosine similarities on CIFAR-10 and CIFAR-100, respectively. (d-f) and (j-l) denote the sample margins on CIFAR-10 and CIFAR-100, respectively.
    }
    \label{fig:cosface-10-cifar10-hist}
    \vskip-10pt
\end{figure}

==> figures/hists/cosface-20.tex <==
\begin{figure}[tbp]
    \centering
    \subfigure[$\mu=0$]{
    \label{cifar10-hist-cosface-20-sim}
    \includegraphics[width=0.8in]{figures/hists/cifar10/cifar10_CosFace_20_0.0_sim.png}
    }
    \subfigure[$\mu=0.5$]{
    \label{cifar10-hist-cosface-20-0.5-sim}
    \includegraphics[width=0.8in]{figures/hists/cifar10/cifar10_CosFace_20_0.5_sim.png}
    }
    \subfigure[$\mu=1$]{
    \label{cifar10-hist-cosface-20-1-sim}
    \includegraphics[width=0.8in]{figures/hists/cifar10/cifar10_CosFace_20_0.5_sim.png}
    }
    \subfigure[$\mu=0$]{
    \label{cifar10-hist-cosface-20-sm}
    \includegraphics[width=0.8in]{figures/hists/cifar10/cifar10_CosFace_20_0.0_sm.png}
    }
    \subfigure[$\mu=0.5$]{
    \label{cifar10-hist-cosface-20-0.5-sm}
    \includegraphics[width=0.8in]{figures/hists/cifar10/cifar10_CosFace_20_0.5_sm.png}
    }
    \subfigure[$\mu=1$]{
    \label{cifar10-hist-cosface-20-1-sm}
    \includegraphics[width=0.8in]{figures/hists/cifar10/cifar10_CosFace_20_0.5_sm.png}
    }
    \subfigure[$\mu=0$]{
    \label{cifar100-hist-cosface-20-sim}
    \includegraphics[width=0.8in]{figures/hists/cifar100/cifar100_CosFace_20_0.0_sim.png}
    }
    \subfigure[$\mu=0.5$]{
    \label{cifar100-hist-cosface-20-0.5-sim}
    \includegraphics[width=0.8in]{figures/hists/cifar100/cifar100_CosFace_20_0.5_sim.png}
    }
    \subfigure[$\mu=1$]{
    \label{cifar100-hist-cosface-20-1-sim}
    \includegraphics[width=0.8in]{figures/hists/cifar100/cifar100_CosFace_20_0.5_sim.png}
    }
    \subfigure[$\mu=0$]{
    \label{cifar100-hist-cosface-20-sm}
    \includegraphics[width=0.8in]{figures/hists/cifar100/cifar100_CosFace_20_0.0_sm.png}
    }
    \subfigure[$\mu=0.5$]{
    \label{cifar100-hist-cosface-20-0.5-sm}
    \includegraphics[width=0.8in]{figures/hists/cifar100/cifar100_CosFace_20_0.5_sm.png}
    }
    \subfigure[$\mu=1$]{
    \label{cifar100-hist-cosface-20-1-sm}
    \includegraphics[width=0.8in]{figures/hists/cifar100/cifar100_CosFace_20_0.5_sm.png}
    }
    \caption{Histogram of similarities and sample margins for CosFace ($s=20$) with/without sample margin regularization $R_{\text{sm}}$ on CIFAR-10 and CIFAR-100. (a-c) and (g-i) denote the cosine similarities on CIFAR-10 and CIFAR-100, respectively. (d-f) and (j-l) denote the sample margins on CIFAR-10 and CIFAR-100, respectively.
    }
    \label{fig:cosface-20-cifar10-hist}
    \vskip-10pt
\end{figure}

==> figures/hists/cosface-40.tex <==
\begin{figure}[tbp]
    \centering
    \subfigure[$\mu=0$]{
    \label{cifar10-hist-cosface-40-sim}
    \includegraphics[width=0.8in]{figures/hists/cifar10/cifar10_CosFace_40_0.0_sim.png}
    }
    \subfigure[$\mu=0.5$]{
    \label{cifar10-hist-cosface-40-0.5-sim}
    \includegraphics[width=0.8in]{figures/hists/cifar10/cifar10_CosFace_40_0.5_sim.png}
    }
    \subfigure[$\mu=1$]{
    \label{cifar10-hist-cosface-40-1-sim}
    \includegraphics[width=0.8in]{figures/hists/cifar10/cifar10_CosFace_40_0.5_sim.png}
    }
    \subfigure[$\mu=0$]{
    \label{cifar10-hist-cosface-40-sm}
    \includegraphics[width=0.8in]{figures/hists/cifar10/cifar10_CosFace_40_0.0_sm.png}
    }
    \subfigure[$\mu=0.5$]{
    \label{cifar10-hist-cosface-40-0.5-sm}
    \includegraphics[width=0.8in]{figures/hists/cifar10/cifar10_CosFace_40_0.5_sm.png}
    }
    \subfigure[$\mu=1$]{
    \label{cifar10-hist-cosface-40-1-sm}
    \includegraphics[width=0.8in]{figures/hists/cifar10/cifar10_CosFace_40_0.5_sm.png}
    }
    \subfigure[$\mu=0$]{
    \label{cifar100-hist-cosface-40-sim}
    \includegraphics[width=0.8in]{figures/hists/cifar100/cifar100_CosFace_40_0.0_sim.png}
    }
    \subfigure[$\mu=0.5$]{
    \label{cifar100-hist-cosface-40-0.5-sim}
    \includegraphics[width=0.8in]{figures/hists/cifar100/cifar100_CosFace_40_0.5_sim.png}
    }
    \subfigure[$\mu=1$]{
    \label{cifar100-hist-cosface-40-1-sim}
    \includegraphics[width=0.8in]{figures/hists/cifar100/cifar100_CosFace_40_0.5_sim.png}
    }
    \subfigure[$\mu=0$]{
    \label{cifar100-hist-cosface-40-sm}
    \includegraphics[width=0.8in]{figures/hists/cifar100/cifar100_CosFace_40_0.0_sm.png}
    }
    \subfigure[$\mu=0.5$]{
    \label{cifar100-hist-cosface-40-0.5-sm}
    \includegraphics[width=0.8in]{figures/hists/cifar100/cifar100_CosFace_40_0.5_sm.png}
    }
    \subfigure[$\mu=1$]{
    \label{cifar100-hist-cosface-40-1-sm}
    \includegraphics[width=0.8in]{figures/hists/cifar100/cifar100_CosFace_40_0.5_sm.png}
    }
    \vskip-10pt
    \caption{Histogram of similarities and sample margins for CosFace ($s=40$) with/without sample margin regularization $R_{\text{sm}}$ on CIFAR-40 and CIFAR-400. (a-c) and (g-i) denote the cosine similarities on CIFAR-40 and CIFAR-400, respectively. (d-f) and (j-l) denote the sample margins on CIFAR-40 and CIFAR-400, respectively.
    }
    \label{fig:cosface-40-cifar10-hist}
    \vskip-40pt
\end{figure}

==> figures/hists/cosface-5.tex <==
\begin{figure}[tbp]
    \centering
    \subfigure[$\mu=0$]{
    \label{cifar10-hist-cosface-5-sim}
    \includegraphics[width=0.8in]{figures/hists/cifar10/cifar10_CosFace_5_0.0_sim.png}
    }
    \subfigure[$\mu=0.5$]{
    \label{cifar10-hist-cosface-5-0.5-sim}
    \includegraphics[width=0.8in]{figures/hists/cifar10/cifar10_CosFace_5_0.5_sim.png}
    }
    \subfigure[$\mu=1$]{
    \label{cifar10-hist-cosface-5-1-sim}
    \includegraphics[width=0.8in]{figures/hists/cifar10/cifar10_CosFace_5_0.5_sim.png}
    }
    \subfigure[$\mu=0$]{
    \label{cifar10-hist-cosface-5-sm}
    \includegraphics[width=0.8in]{figures/hists/cifar10/cifar10_CosFace_5_0.0_sm.png}
    }
    \subfigure[$\mu=0.5$]{
    \label{cifar10-hist-cosface-5-0.5-sm}
    \includegraphics[width=0.8in]{figures/hists/cifar10/cifar10_CosFace_5_0.5_sm.png}
    }
    \subfigure[$\mu=1$]{
    \label{cifar10-hist-cosface-5-1-sm}
    \includegraphics[width=0.8in]{figures/hists/cifar10/cifar10_CosFace_5_0.5_sm.png}
    }
    \subfigure[$\mu=0$]{
    \label{cifar100-hist-cosface-5-sim}
    \includegraphics[width=0.8in]{figures/hists/cifar100/cifar100_CosFace_5_0.0_sim.png}
    }
    \subfigure[$\mu=0.5$]{
    \label{cifar100-hist-cosface-5-0.5-sim}
    \includegraphics[width=0.8in]{figures/hists/cifar100/cifar100_CosFace_5_0.5_sim.png}
    }
    \subfigure[$\mu=1$]{
    \label{cifar100-hist-cosface-5-1-sim}
    \includegraphics[width=0.8in]{figures/hists/cifar100/cifar100_CosFace_5_0.5_sim.png}
    }
    \subfigure[$\mu=0$]{
    \label{cifar100-hist-cosface-5-sm}
    \includegraphics[width=0.8in]{figures/hists/cifar100/cifar100_CosFace_5_0.0_sm.png}
    }
    \subfigure[$\mu=0.5$]{
    \label{cifar100-hist-cosface-5-0.5-sm}
    \includegraphics[width=0.8in]{figures/hists/cifar100/cifar100_CosFace_5_0.5_sm.png}
    }
    \subfigure[$\mu=1$]{
    \label{cifar100-hist-cosface-5-1-sm}
    \includegraphics[width=0.8in]{figures/hists/cifar100/cifar100_CosFace_5_0.5_sm.png}
    }
    \caption{Histogram of similarities and sample margins for CosFace ($s=15$) with/without sample margin regularization $R_{\text{sm}}$ on CIFAR-10 and CIFAR-100. (a-c) and (g-i) denote the cosine similarities on CIFAR-10 and CIFAR-100, respectively. (d-f) and (j-l) denote the sample margins on CIFAR-10 and CIFAR-100, respectively.
    }
    \label{fig:cosface-5-cifar10-hist}
    \vskip-10pt
\end{figure}

==> figures/hists/imb-step-cifar10-arcface.tex <==
\begin{figure}[tbp]
    \centering
    \subfigure[$\lambda=0$]{
    \label{step-cifar10-hist-arcface-0-sim}
    \includegraphics[width=0.8in]{figures/hists/imb/cifar10_ArcFace_5_step_0.1_0.0_sim.png}
    }
    \subfigure[$\lambda=1$]{
    \label{step-cifar10-hist-arcface-1-sim}
    \includegraphics[width=0.8in]{figures/hists/imb/cifar10_ArcFace_5_step_0.1_1.0_sim.png}
    }
    \subfigure[$\lambda=2$]{
    \label{step-cifar10-hist-arcface-2-sim}
    \includegraphics[width=0.8in]{figures/hists/imb/cifar10_ArcFace_5_step_0.1_2.0_sim.png}
    }
    \subfigure[$\lambda=5$]{
    \label{step-cifar10-hist-arcface-5-sim}
    \includegraphics[width=0.8in]{figures/hists/imb/cifar10_ArcFace_5_step_0.1_5.0_sim.png}
    }
    \subfigure[$\lambda=10$]{
    \label{step-cifar10-hist-arcface-10-sim}
    \includegraphics[width=0.8in]{figures/hists/imb/cifar10_ArcFace_5_step_0.1_10.0_sim.png}
    }
    \subfigure[$\lambda=20$]{
    \label{step-cifar10-hist-arcface-20-sim}
    \includegraphics[width=0.8in]{figures/hists/imb/cifar10_ArcFace_5_step_0.1_20.0_sim.png}
    }
    \subfigure[$\lambda=0$]{
    \label{step-cifar10-hist-arcface-0-sm}
    \includegraphics[width=0.8in]{figures/hists/imb/cifar10_ArcFace_5_step_0.1_0.0_sm.png}
    }
    \subfigure[$\lambda=1$]{
    \label{step-cifar10-hist-arcface-1-sm}
    \includegraphics[width=0.8in]{figures/hists/imb/cifar10_ArcFace_5_step_0.1_1.0_sm.png}
    }
    \subfigure[$\lambda=2$]{
    \label{step-cifar10-hist-arcface-2-sm}
    \includegraphics[width=0.8in]{figures/hists/imb/cifar10_ArcFace_5_step_0.1_2.0_sm.png}
    }
    \subfigure[$\lambda=5$]{
    \label{step-cifar10-hist-arcface-5-sm}
    \includegraphics[width=0.8in]{figures/hists/imb/cifar10_ArcFace_5_step_0.1_5.0_sm.png}
    }
    \subfigure[$\lambda=10$]{
    \label{step-cifar10-hist-arcface-10-sm}
    \includegraphics[width=0.8in]{figures/hists/imb/cifar10_ArcFace_5_step_0.1_10.0_sm.png}
    }
    \subfigure[$\lambda=20$]{
    \label{step-cifar10-hist-arcface-20-sm}
    \includegraphics[width=0.8in]{figures/hists/imb/cifar10_ArcFace_5_step_0.1_20.0_sm.png}
    }

    
    \caption{Histogram of similarities and sample margins for ArcFace using the zero-centroid regularization with different $\lambda$ on step imbalanced CIFAR-10 with $\rho=10$. (a-f) denote the cosine similarities between samples and their corresponding prototypes, and (g-l) denote the sample margins.
    }
    \label{fig:arcface-5-step-cifar10-hist}
    \vskip-10pt
\end{figure}

==> figures/hists/imb-step-cifar10-cosface.tex <==
\begin{figure}[tbp]
    \centering
    \subfigure[$\lambda=0$]{
    \label{exp-cifar10-hist-cosface-0-sim}
    \includegraphics[width=0.8in]{figures/hists/imb/cifar10_CosFace_5_exp_0.1_0.0_sim.png}
    }
    \subfigure[$\lambda=1$]{
    \label{exp-cifar10-hist-cosface-1-sim}
    \includegraphics[width=0.8in]{figures/hists/imb/cifar10_CosFace_5_exp_0.1_1.0_sim.png}
    }
    \subfigure[$\lambda=2$]{
    \label{exp-cifar10-hist-cosface-2-sim}
    \includegraphics[width=0.8in]{figures/hists/imb/cifar10_CosFace_5_exp_0.1_2.0_sim.png}
    }
    \subfigure[$\lambda=5$]{
    \label{exp-cifar10-hist-cosface-5-sim}
    \includegraphics[width=0.8in]{figures/hists/imb/cifar10_CosFace_5_exp_0.1_5.0_sim.png}
    }
    \subfigure[$\lambda=10$]{
    \label{exp-cifar10-hist-cosface-10-sim}
    \includegraphics[width=0.8in]{figures/hists/imb/cifar10_CosFace_5_exp_0.1_10.0_sim.png}
    }
    \subfigure[$\lambda=20$]{
    \label{exp-cifar10-hist-cosface-20-sim}
    \includegraphics[width=0.8in]{figures/hists/imb/cifar10_CosFace_5_exp_0.1_20.0_sim.png}
    }
    \subfigure[$\lambda=0$]{
    \label{exp-cifar10-hist-cosface-0-sm}
    \includegraphics[width=0.8in]{figures/hists/imb/cifar10_CosFace_5_exp_0.1_0.0_sm.png}
    }
    \subfigure[$\lambda=1$]{
    \label{exp-cifar10-hist-cosface-1-sm}
    \includegraphics[width=0.8in]{figures/hists/imb/cifar10_CosFace_5_exp_0.1_1.0_sm.png}
    }
    \subfigure[$\lambda=2$]{
    \label{exp-cifar10-hist-cosface-2-sm}
    \includegraphics[width=0.8in]{figures/hists/imb/cifar10_CosFace_5_exp_0.1_2.0_sm.png}
    }
    \subfigure[$\lambda=5$]{
    \label{exp-cifar10-hist-cosface-5-sm}
    \includegraphics[width=0.8in]{figures/hists/imb/cifar10_CosFace_5_exp_0.1_5.0_sm.png}
    }
    \subfigure[$\lambda=10$]{
    \label{exp-cifar10-hist-cosface-10-sm}
    \includegraphics[width=0.8in]{figures/hists/imb/cifar10_CosFace_5_exp_0.1_10.0_sm.png}
    }
    \subfigure[$\lambda=20$]{
    \label{exp-cifar10-hist-cosface-20-sm}
    \includegraphics[width=0.8in]{figures/hists/imb/cifar10_CosFace_5_exp_0.1_20.0_sm.png}
    }

    
    \caption{Histogram of similarities and sample margins for CosFace using the zero-centroid regularization with different $\lambda$ on long-tailed imbalanced CIFAR-10 with $\rho=10$. (a-f) denote the cosine similarities between samples and their corresponding prototypes, and (g-l) denote the sample margins.
    }
    \label{fig:cosface-5-exp-cifar10-hist}
    \vskip-10pt
\end{figure}

==> figures/hists/imb-step-cifar10-ldam.tex <==
\begin{figure}[tbp]
    \centering
    \subfigure[$\lambda=0$]{
    \label{exp-cifar10-hist-ldam-0-sim}
    \includegraphics[width=0.8in]{figures/hists/imb/cifar10_LDAM_5_exp_0.1_0.0_sim.png}
    }
    \subfigure[$\lambda=1$]{
    \label{exp-cifar10-hist-ldam-1-sim}
    \includegraphics[width=0.8in]{figures/hists/imb/cifar10_LDAM_5_exp_0.1_1.0_sim.png}
    }
    \subfigure[$\lambda=2$]{
    \label{exp-cifar10-hist-ldam-2-sim}
    \includegraphics[width=0.8in]{figures/hists/imb/cifar10_LDAM_5_exp_0.1_2.0_sim.png}
    }
    \subfigure[$\lambda=5$]{
    \label{exp-cifar10-hist-ldam-5-sim}
    \includegraphics[width=0.8in]{figures/hists/imb/cifar10_LDAM_5_exp_0.1_5.0_sim.png}
    }
    \subfigure[$\lambda=10$]{
    \label{exp-cifar10-hist-ldam-10-sim}
    \includegraphics[width=0.8in]{figures/hists/imb/cifar10_LDAM_5_exp_0.1_10.0_sim.png}
    }
    \subfigure[$\lambda=20$]{
    \label{exp-cifar10-hist-ldam-20-sim}
    \includegraphics[width=0.8in]{figures/hists/imb/cifar10_LDAM_5_exp_0.1_20.0_sim.png}
    }
    \subfigure[$\lambda=0$]{
    \label{exp-cifar10-hist-ldam-0-sm}
    \includegraphics[width=0.8in]{figures/hists/imb/cifar10_LDAM_5_exp_0.1_0.0_sm.png}
    }
    \subfigure[$\lambda=1$]{
    \label{exp-cifar10-hist-ldam-1-sm}
    \includegraphics[width=0.8in]{figures/hists/imb/cifar10_LDAM_5_exp_0.1_1.0_sm.png}
    }
    \subfigure[$\lambda=2$]{
    \label{exp-cifar10-hist-ldam-2-sm}
    \includegraphics[width=0.8in]{figures/hists/imb/cifar10_LDAM_5_exp_0.1_2.0_sm.png}
    }
    \subfigure[$\lambda=5$]{
    \label{exp-cifar10-hist-ldam-5-sm}
    \includegraphics[width=0.8in]{figures/hists/imb/cifar10_LDAM_5_exp_0.1_5.0_sm.png}
    }
    \subfigure[$\lambda=10$]{
    \label{exp-cifar10-hist-ldam-10-sm}
    \includegraphics[width=0.8in]{figures/hists/imb/cifar10_LDAM_5_exp_0.1_10.0_sm.png}
    }
    \subfigure[$\lambda=20$]{
    \label{exp-cifar10-hist-ldam-20-sm}
    \includegraphics[width=0.8in]{figures/hists/imb/cifar10_LDAM_5_exp_0.1_20.0_sm.png}
    }

    
    \caption{Histogram of similarities and sample margins for LDAM using the zero-centroid regularization with different $\lambda$ on long-tailed imbalanced CIFAR-10 with $\rho=10$. (a-f) denote the cosine similarities between samples and their corresponding prototypes, and (g-l) denote the sample margins.
    }
    \label{fig:ldam-5-exp-cifar10-hist}
    \vskip-10pt
\end{figure}

==> figures/hists/imb-step-cifar10-normface.tex <==
\begin{figure}[tbp]
    \centering
    \subfigure[$\lambda=0$]{
    \label{step-cifar10-hist-normface-0-sim}
    \includegraphics[width=0.8in]{figures/hists/imb/cifar10_Norm_5_step_0.1_0.0_sim.png}
    }
    \subfigure[$\lambda=1$]{
    \label{step-cifar10-hist-normface-1-sim}
    \includegraphics[width=0.8in]{figures/hists/imb/cifar10_Norm_5_step_0.1_1.0_sim.png}
    }
    \subfigure[$\lambda=2$]{
    \label{step-cifar10-hist-normface-2-sim}
    \includegraphics[width=0.8in]{figures/hists/imb/cifar10_Norm_5_step_0.1_2.0_sim.png}
    }
    \subfigure[$\lambda=5$]{
    \label{step-cifar10-hist-normface-5-sim}
    \includegraphics[width=0.8in]{figures/hists/imb/cifar10_Norm_5_step_0.1_5.0_sim.png}
    }
    \subfigure[$\lambda=10$]{
    \label{step-cifar10-hist-normface-10-sim}
    \includegraphics[width=0.8in]{figures/hists/imb/cifar10_Norm_5_step_0.1_10.0_sim.png}
    }
    \subfigure[$\lambda=20$]{
    \label{step-cifar10-hist-normface-20-sim}
    \includegraphics[width=0.8in]{figures/hists/imb/cifar10_Norm_5_step_0.1_20.0_sim.png}
    }
    \subfigure[$\lambda=0$]{
    \label{step-cifar10-hist-normface-0-sm}
    \includegraphics[width=0.8in]{figures/hists/imb/cifar10_Norm_5_step_0.1_0.0_sm.png}
    }
    \subfigure[$\lambda=1$]{
    \label{step-cifar10-hist-normface-1-sm}
    \includegraphics[width=0.8in]{figures/hists/imb/cifar10_Norm_5_step_0.1_1.0_sm.png}
    }
    \subfigure[$\lambda=2$]{
    \label{step-cifar10-hist-normface-2-sm}
    \includegraphics[width=0.8in]{figures/hists/imb/cifar10_Norm_5_step_0.1_2.0_sm.png}
    }
    \subfigure[$\lambda=5$]{
    \label{step-cifar10-hist-normface-5-sm}
    \includegraphics[width=0.8in]{figures/hists/imb/cifar10_Norm_5_step_0.1_5.0_sm.png}
    }
    \subfigure[$\lambda=10$]{
    \label{step-cifar10-hist-normface-10-sm}
    \includegraphics[width=0.8in]{figures/hists/imb/cifar10_Norm_5_step_0.1_10.0_sm.png}
    }
    \subfigure[$\lambda=20$]{
    \label{step-cifar10-hist-normface-20-sm}
    \includegraphics[width=0.8in]{figures/hists/imb/cifar10_Norm_5_step_0.1_20.0_sm.png}
    }

    
    \caption{Histogram of similarities and sample margins for NormFace using the zero-centroid regularization with different $\lambda$ on step imbalanced CIFAR-10 with $\rho=10$. (a-f) denote the cosine similarities between samples and their corresponding prototypes, and (g-l) denote the sample margins.
    }
    \label{fig:normface-5-step-cifar10-hist}
    \vskip-10pt
\end{figure}

==> figures/hists/normface-10.tex <==
\begin{figure}[tbp]
    \centering
    \subfigure[$\mu=0$]{
    \label{cifar10-hist-normface-10-sim}
    \includegraphics[width=0.8in]{figures/hists/cifar10/cifar10_Norm_10_0.0_sim.png}
    }
    \subfigure[$\mu=0.5$]{
    \label{cifar10-hist-normface-10-0.5-sim}
    \includegraphics[width=0.8in]{figures/hists/cifar10/cifar10_Norm_10_0.5_sim.png}
    }
    \subfigure[$\mu=1$]{
    \label{cifar10-hist-normface-10-1-sim}
    \includegraphics[width=0.8in]{figures/hists/cifar10/cifar10_Norm_10_0.5_sim.png}
    }
    \subfigure[$\mu=0$]{
    \label{cifar10-hist-normface-10-sm}
    \includegraphics[width=0.8in]{figures/hists/cifar10/cifar10_Norm_10_0.0_sm.png}
    }
    \subfigure[$\mu=0.5$]{
    \label{cifar10-hist-normface-10-0.5-sm}
    \includegraphics[width=0.8in]{figures/hists/cifar10/cifar10_Norm_10_0.5_sm.png}
    }
    \subfigure[$\mu=1$]{
    \label{cifar10-hist-normface-10-1-sm}
    \includegraphics[width=0.8in]{figures/hists/cifar10/cifar10_Norm_10_0.5_sm.png}
    }
    \subfigure[$\mu=0$]{
    \label{cifar100-hist-normface-10-sim}
    \includegraphics[width=0.8in]{figures/hists/cifar100/cifar100_Norm_10_0.0_sim.png}
    }
    \subfigure[$\mu=0.5$]{
    \label{cifar100-hist-normface-10-0.5-sim}
    \includegraphics[width=0.8in]{figures/hists/cifar100/cifar100_Norm_10_0.5_sim.png}
    }
    \subfigure[$\mu=1$]{
    \label{cifar100-hist-normface-10-1-sim}
    \includegraphics[width=0.8in]{figures/hists/cifar100/cifar100_Norm_10_0.5_sim.png}
    }
    \subfigure[$\mu=0$]{
    \label{cifar100-hist-normface-10-sm}
    \includegraphics[width=0.8in]{figures/hists/cifar100/cifar100_Norm_10_0.0_sm.png}
    }
    \subfigure[$\mu=0.5$]{
    \label{cifar100-hist-normface-10-0.5-sm}
    \includegraphics[width=0.8in]{figures/hists/cifar100/cifar100_Norm_10_0.5_sm.png}
    }
    \subfigure[$\mu=1$]{
    \label{cifar100-hist-normface-10-1-sm}
    \includegraphics[width=0.8in]{figures/hists/cifar100/cifar100_Norm_10_0.5_sm.png}
    }
    \caption{Histogram of similarities and sample margins for NormFace ($s=10$) with/without sample margin regularization $R_{\text{sm}}$ on CIFAR-10 and CIFAR-100. (a-c) and (g-i) denote the cosine similarities on CIFAR-10 and CIFAR-100, respectively. (d-f) and (j-l) denote the sample margins on CIFAR-10 and CIFAR-100, respectively.
    }
    \label{fig:normface-10-cifar10-hist}
    \vskip-10pt
\end{figure}

==> figures/hists/normface-20.tex <==
\begin{figure}[tbp]
    \centering
    \subfigure[$\mu=0$]{
    \label{cifar10-hist-normface-5-sim}
    \includegraphics[width=0.8in]{figures/hists/cifar10/cifar10_Norm_20_0.0_sim.png}
    }
    \subfigure[$\mu=0.5$]{
    \label{cifar10-hist-normface-5-0.5-sim}
    \includegraphics[width=0.8in]{figures/hists/cifar10/cifar10_Norm_20_0.5_sim.png}
    }
    \subfigure[$\mu=1$]{
    \label{cifar10-hist-normface-5-1-sim}
    \includegraphics[width=0.8in]{figures/hists/cifar10/cifar10_Norm_20_0.5_sim.png}
    }
    \subfigure[$\mu=0$]{
    \label{cifar10-hist-normface-5-sm}
    \includegraphics[width=0.8in]{figures/hists/cifar10/cifar10_Norm_20_0.0_sm.png}
    }
    \subfigure[$\mu=0.5$]{
    \label{cifar10-hist-normface-5-0.5-sm}
    \includegraphics[width=0.8in]{figures/hists/cifar10/cifar10_Norm_20_0.5_sm.png}
    }
    \subfigure[$\mu=1$]{
    \label{cifar10-hist-normface-5-1-sm}
    \includegraphics[width=0.8in]{figures/hists/cifar10/cifar10_Norm_20_0.5_sm.png}
    }
    \subfigure[$\mu=0$]{
    \label{cifar100-hist-normface-5-sim}
    \includegraphics[width=0.8in]{figures/hists/cifar100/cifar100_Norm_20_0.0_sim.png}
    }
    \subfigure[$\mu=0.5$]{
    \label{cifar100-hist-normface-5-0.5-sim}
    \includegraphics[width=0.8in]{figures/hists/cifar100/cifar100_Norm_20_0.5_sim.png}
    }
    \subfigure[$\mu=1$]{
    \label{cifar100-hist-normface-5-1-sim}
    \includegraphics[width=0.8in]{figures/hists/cifar100/cifar100_Norm_20_0.5_sim.png}
    }
    \subfigure[$\mu=0$]{
    \label{cifar100-hist-normface-5-sm}
    \includegraphics[width=0.8in]{figures/hists/cifar100/cifar100_Norm_20_0.0_sm.png}
    }
    \subfigure[$\mu=0.5$]{
    \label{cifar100-hist-normface-5-0.5-sm}
    \includegraphics[width=0.8in]{figures/hists/cifar100/cifar100_Norm_20_0.5_sm.png}
    }
    \subfigure[$\mu=1$]{
    \label{cifar100-hist-normface-5-1-sm}
    \includegraphics[width=0.8in]{figures/hists/cifar100/cifar100_Norm_20_0.5_sm.png}
    }
    \caption{Histogram of similarities and sample margins for NormFace ($s=20$) with/without sample margin regularization $R_{\text{sm}}$ on CIFAR-10 and CIFAR-100. (a-c) and (g-i) denote the cosine similarities on CIFAR-10 and CIFAR-100, respectively. (d-f) and (j-l) denote the sample margins on CIFAR-10 and CIFAR-100, respectively.
    }
    \label{fig:normface-5-cifar10-hist}
    \vskip-10pt
\end{figure}

==> figures/hists/normface-40.tex <==
\begin{figure}[tbp]
    \centering
    \subfigure[$\mu=0$]{
    \label{cifar10-hist-normface-10-sim}
    \includegraphics[width=0.8in]{figures/hists/cifar10/cifar10_Norm_40_0.0_sim.png}
    }
    \subfigure[$\mu=0.5$]{
    \label{cifar10-hist-normface-10-0.5-sim}
    \includegraphics[width=0.8in]{figures/hists/cifar10/cifar10_Norm_40_0.5_sim.png}
    }
    \subfigure[$\mu=1$]{
    \label{cifar10-hist-normface-10-1-sim}
    \includegraphics[width=0.8in]{figures/hists/cifar10/cifar10_Norm_40_0.5_sim.png}
    }
    \subfigure[$\mu=0$]{
    \label{cifar10-hist-normface-10-sm}
    \includegraphics[width=0.8in]{figures/hists/cifar10/cifar10_Norm_40_0.0_sm.png}
    }
    \subfigure[$\mu=0.5$]{
    \label{cifar10-hist-normface-10-0.5-sm}
    \includegraphics[width=0.8in]{figures/hists/cifar10/cifar10_Norm_40_0.5_sm.png}
    }
    \subfigure[$\mu=1$]{
    \label{cifar10-hist-normface-10-1-sm}
    \includegraphics[width=0.8in]{figures/hists/cifar10/cifar10_Norm_40_0.5_sm.png}
    }
    \subfigure[$\mu=0$]{
    \label{cifar100-hist-normface-10-sim}
    \includegraphics[width=0.8in]{figures/hists/cifar100/cifar100_Norm_40_0.0_sim.png}
    }
    \subfigure[$\mu=0.5$]{
    \label{cifar100-hist-normface-10-0.5-sim}
    \includegraphics[width=0.8in]{figures/hists/cifar100/cifar100_Norm_40_0.5_sim.png}
    }
    \subfigure[$\mu=1$]{
    \label{cifar100-hist-normface-10-1-sim}
    \includegraphics[width=0.8in]{figures/hists/cifar100/cifar100_Norm_40_0.5_sim.png}
    }
    \subfigure[$\mu=0$]{
    \label{cifar100-hist-normface-10-sm}
    \includegraphics[width=0.8in]{figures/hists/cifar100/cifar100_Norm_40_0.0_sm.png}
    }
    \subfigure[$\mu=0.5$]{
    \label{cifar100-hist-normface-10-0.5-sm}
    \includegraphics[width=0.8in]{figures/hists/cifar100/cifar100_Norm_40_0.5_sm.png}
    }
    \subfigure[$\mu=1$]{
    \label{cifar100-hist-normface-10-1-sm}
    \includegraphics[width=0.8in]{figures/hists/cifar100/cifar100_Norm_40_0.5_sm.png}
    }
    \caption{Histogram of similarities and sample margins for NormFace ($s=40$) with/without sample margin regularization $R_{\text{sm}}$ on CIFAR-10 and CIFAR-100. (a-c) and (g-i) denote the cosine similarities on CIFAR-10 and CIFAR-100, respectively. (d-f) and (j-l) denote the sample margins on CIFAR-10 and CIFAR-100, respectively.
    }
    \label{fig:normface-10-cifar10-hist}
    \vskip-10pt
\end{figure}

==> figures/hists/normface-5.tex <==
\begin{figure}[tbp]
    \centering
    \subfigure[$\mu=0$]{
    \label{cifar10-hist-normface-5-sim}
    \includegraphics[width=0.8in]{figures/hists/cifar10/cifar10_Norm_5_0.0_sim.png}
    }
    \subfigure[$\mu=0.5$]{
    \label{cifar10-hist-normface-5-0.5-sim}
    \includegraphics[width=0.8in]{figures/hists/cifar10/cifar10_Norm_5_0.5_sim.png}
    }
    \subfigure[$\mu=1$]{
    \label{cifar10-hist-normface-5-1-sim}
    \includegraphics[width=0.8in]{figures/hists/cifar10/cifar10_Norm_5_0.5_sim.png}
    }
    \subfigure[$\mu=0$]{
    \label{cifar10-hist-normface-5-sm}
    \includegraphics[width=0.8in]{figures/hists/cifar10/cifar10_Norm_5_0.0_sm.png}
    }
    \subfigure[$\mu=0.5$]{
    \label{cifar10-hist-normface-5-0.5-sm}
    \includegraphics[width=0.8in]{figures/hists/cifar10/cifar10_Norm_5_0.5_sm.png}
    }
    \subfigure[$\mu=1$]{
    \label{cifar10-hist-normface-5-1-sm}
    \includegraphics[width=0.8in]{figures/hists/cifar10/cifar10_Norm_5_0.5_sm.png}
    }
    \subfigure[$\mu=0$]{
    \label{cifar100-hist-normface-5-sim}
    \includegraphics[width=0.8in]{figures/hists/cifar100/cifar100_Norm_5_0.0_sim.png}
    }
    \subfigure[$\mu=0.5$]{
    \label{cifar100-hist-normface-5-0.5-sim}
    \includegraphics[width=0.8in]{figures/hists/cifar100/cifar100_Norm_5_0.5_sim.png}
    }
    \subfigure[$\mu=1$]{
    \label{cifar100-hist-normface-5-1-sim}
    \includegraphics[width=0.8in]{figures/hists/cifar100/cifar100_Norm_5_0.5_sim.png}
    }
    \subfigure[$\mu=0$]{
    \label{cifar100-hist-normface-5-sm}
    \includegraphics[width=0.8in]{figures/hists/cifar100/cifar100_Norm_5_0.0_sm.png}
    }
    \subfigure[$\mu=0.5$]{
    \label{cifar100-hist-normface-5-0.5-sm}
    \includegraphics[width=0.8in]{figures/hists/cifar100/cifar100_Norm_5_0.5_sm.png}
    }
    \subfigure[$\mu=1$]{
    \label{cifar100-hist-normface-5-1-sm}
    \includegraphics[width=0.8in]{figures/hists/cifar100/cifar100_Norm_5_0.5_sm.png}
    }
    \caption{Histogram of similarities and sample margins for NormFace ($s=5$) with/without sample margin regularization $R_{\text{sm}}$ on CIFAR-10 and CIFAR-100. (a-c) and (g-i) denote the cosine similarities on CIFAR-10 and CIFAR-100, respectively. (d-f) and (j-l) denote the sample margins on CIFAR-10 and CIFAR-100, respectively.
    }
    \label{fig:normface-5-cifar10-hist}
    \vskip-10pt
\end{figure}

==> tables/full_fav.tex <==
\begin{tabular}{l|cccc}
    \toprule
    Method & best acc & acc & top1 & top5\\
    \midrule
    CosFace & 97.90 & 97.57 & 79.69 & 94.95\\
    ArcFace & 97.81 & 97.38 & - & -\\
    NormFace & 95.80 & 95.75 & 57.57 & 69.35\\
    \textbf{CosFace*} (0.5) & 98.08 & 97.58 & 81.47 & 86.40\\
    \textbf{ArcFace*} (0.5) & 98.18 & 97.45 & 80.51 & 85.54\\
    \textbf{NormFace*} (0.5) & 96.23 & 96.18 & 60.11 & 71.44\\
    \textbf{LM-Softmax} & \textbf{98.35} & \textbf{97.62} & 81.28 & 86.04\\
    
     \bottomrule
\end{tabular}

==> tables/imb_cifar10.tex <==

\begin{table}[htbp]
    \caption{Test accuracies and class margins on imbalanced CIFAR-10.}
    \label{im-cifar10}
    \centering
    \begin{tabular}{l|cc|cc|cc|cc}
        \toprule
         Imbalance Type &  \multicolumn{4}{c|}{long-tailed} & \multicolumn{4}{c}{step}\\
         \midrule
         Imbalance Ratio &  \multicolumn{2}{c|}{100} & \multicolumn{2}{c|}{10} & \multicolumn{2}{c|}{100} & \multicolumn{2}{c}{10}\\
         \midrule
         Metric & acc & cls\_ m & acc & cls\_ m & acc & cls\_ m & acc & cls\_ m\\
         \midrule
         CE & 70.88 & 87.41$^\circ$ & 88.17 & 79.63$^\circ$ & 64.21 & 76.50$^\circ$ & 85.06 & 82.24$^\circ$\\
         Focal & 66.30 & 74.14$^\circ$ & 87.33 & 74.48$^\circ$ & 60.55 & 63.30$^\circ$ & 84.49 & 75.16$^\circ$\\
         \midrule
         CosFace ($\lambda=0$) & 69.28 & 58.77$^\circ$ & 87.02 & 81.61$^\circ$ & 53.64 & 19.78$^\circ$ & 84.86 & 75.96$^\circ$\\ 
        CosFace ($\lambda=1$) & 68.86 & \textbf{96.17$^\circ$} & \textbf{87.24} & \textbf{96.16$^\circ$} & \textbf{62.24} & \textbf{95.93$^\circ$} & \textbf{84.98} & \textbf{96.26$^\circ$}\\ 
        CosFace ($\lambda=2$) & \textbf{69.40} & \textbf{95.61$^\circ$} & \textbf{87.16} & \textbf{96.26$^\circ$} & \textbf{62.49} & \textbf{95.86$^\circ$} & 84.69 & \textbf{95.88$^\circ$}\\ 
        CosFace ($\lambda=5$) & 69.18 & \textbf{93.73$^\circ$} & \textbf{87.34} & \textbf{96.24$^\circ$} & \textbf{62.13} & \textbf{95.84$^\circ$} & \textbf{85.07} & \textbf{96.24$^\circ$}\\ 
        CosFace ($\lambda=10$) & 68.83 & \textbf{92.49$^\circ$} & 86.94 & \textbf{96.23$^\circ$} & \textbf{61.99} & \textbf{95.35$^\circ$} & \textbf{85.59} & \textbf{96.12$^\circ$}\\ 
        CosFace ($\lambda=20$) & \textbf{69.52} & \textbf{91.90$^\circ$} & \textbf{87.55} & \textbf{95.46$^\circ$} & \textbf{62.38} & \textbf{94.36$^\circ$} & \textbf{85.15} & \textbf{95.88$^\circ$}\\ 
        \midrule
        ArcFace ($\lambda=0$) & 72.20 & 65.86$^\circ$ & 89.00 & 85.23$^\circ$ & 62.48 & 54.29$^\circ$ & 86.32 & 80.51$^\circ$\\ 
        ArcFace ($\lambda=1$) & 71.69 & \textbf{95.08$^\circ$} & 88.86 & \textbf{96.26$^\circ$} & \textbf{63.10} & \textbf{95.83$^\circ$} & \textbf{86.49} & \textbf{96.23$^\circ$}\\ 
        ArcFace ($\lambda=2$) & 71.91 & \textbf{93.78$^\circ$} & 88.78 & \textbf{96.24$^\circ$} & \textbf{63.05} & \textbf{94.84$^\circ$} & 86.18 & \textbf{96.23$^\circ$}\\ 
        ArcFace ($\lambda=5$) & \textbf{72.23} & \textbf{92.30$^\circ$} & \textbf{89.22} & \textbf{96.23$^\circ$} & \textbf{64.38} & \textbf{95.01$^\circ$} & \textbf{86.56} & \textbf{96.24$^\circ$}\\ 
        ArcFace ($\lambda=10$) & 71.99 & \textbf{91.92$^\circ$} & 88.99 & \textbf{94.68$^\circ$} & \textbf{63.59} & \textbf{94.97$^\circ$} & \textbf{86.65} & \textbf{96.23$^\circ$}\\ 
        ArcFace ($\lambda=20$) & 71.75 & \textbf{91.42$^\circ$} & 88.99 & \textbf{92.85$^\circ$} & \textbf{63.56} & \textbf{93.29$^\circ$} & 86.15 & \textbf{95.83$^\circ$}\\ 
        \midrule
        NormFace ($\lambda=0$) & 72.37 & 62.72$^\circ$ & 89.19 & 82.60$^\circ$ & 63.69 & 51.00$^\circ$ & 86.37 & 77.82$^\circ$\\ 
        NormFace ($\lambda=1$) & 72.07 & \textbf{94.95$^\circ$} & 89.18 & \textbf{96.27$^\circ$} & 62.40 & \textbf{96.15$^\circ$} & \textbf{86.46} & \textbf{96.29$^\circ$}\\ 
        NormFace ($\lambda=2$) & 71.92 & \textbf{94.29$^\circ$} & 88.93 & \textbf{96.28$^\circ$} & 63.21 & \textbf{96.14$^\circ$} & 86.26 & \textbf{96.30$^\circ$}\\ 
        NormFace ($\lambda=5$) & 70.79 & \textbf{92.37$^\circ$} & 88.84 & \textbf{96.17$^\circ$} & 62.83 & \textbf{95.38$^\circ$} & \textbf{86.49} & \textbf{96.28$^\circ$}\\ 
        NormFace ($\lambda=10$) & 72.04 & \textbf{91.95$^\circ$} & \textbf{89.30} & \textbf{94.50$^\circ$} & 63.45 & \textbf{94.75$^\circ$} & 86.06 & \textbf{96.29$^\circ$}\\ 
        NormFace ($\lambda=20$) & 71.36 & \textbf{91.14$^\circ$} & 89.08 & \textbf{93.40$^\circ$} & \textbf{64.07} & \textbf{93.06$^\circ$} & \textbf{86.50} & \textbf{95.94$^\circ$}\\ 
        \midrule
        LDAM ($\lambda=0$) & 72.86 & 73.30$^\circ$ & 88.92 & 88.19$^\circ$ & 63.27 & 61.42$^\circ$ & 87.04 & 85.21$^\circ$\\ 
        LDAM ($\lambda=1$) & 72.50 & \textbf{96.25$^\circ$} & \textbf{88.97} & \textbf{96.24$^\circ$} & \textbf{64.31} & \textbf{96.10$^\circ$} & 86.74 & \textbf{96.26$^\circ$}\\ 
        LDAM ($\lambda=2$) & 72.41 & \textbf{95.85$^\circ$} & \textbf{89.01} & \textbf{96.24$^\circ$} & \textbf{64.99} & \textbf{96.04$^\circ$} & 86.55 & \textbf{96.28$^\circ$}\\ 
        LDAM ($\lambda=5$) & 71.99 & \textbf{93.83$^\circ$} & \textbf{89.51} & \textbf{96.25$^\circ$} & \textbf{64.79} & \textbf{96.12$^\circ$} & 86.62 & \textbf{96.16$^\circ$}\\ 
        LDAM ($\lambda=10$) & 72.21 & \textbf{92.49$^\circ$} & 88.92 & \textbf{96.18$^\circ$} & \textbf{64.48} & \textbf{96.16$^\circ$} & 86.69 & \textbf{96.29$^\circ$}\\ 
        LDAM ($\lambda=20$) & 72.86 & \textbf{91.75$^\circ$} & \textbf{89.20} & \textbf{95.59$^\circ$} & \textbf{64.66} & \textbf{94.55$^\circ$} & 86.60 & \textbf{96.05$^\circ$}\\ 
        \midrule
        LM-Softmax ($\lambda=0$) & 65.32 & 4.42$^\circ$ & 88.69 & 68.91$^\circ$ & 50.47 & 0.45$^\circ$ & 86.08 & 52.20$^\circ$\\ 
        LM-Softmax ($\lambda=1$) & \textbf{72.25} & \textbf{96.06$^\circ$} & 88.47 & \textbf{96.26$^\circ$} & \textbf{64.18} & \textbf{91.44$^\circ$} & \textbf{86.66} & \textbf{96.14$^\circ$}\\ 
        LM-Softmax ($\lambda=2$) & \textbf{72.57} & \textbf{95.83$^\circ$} & 88.69 & \textbf{96.31$^\circ$} & \textbf{65.58} & \textbf{93.23$^\circ$} & \textbf{86.70} & \textbf{96.11$^\circ$}\\ 
        LM-Softmax ($\lambda=5$) & \textbf{72.53} & \textbf{93.65$^\circ$} & 88.60 & \textbf{96.26$^\circ$} & \textbf{65.18} & \textbf{95.20$^\circ$} & \textbf{87.07} & \textbf{96.05$^\circ$}\\ 
        LM-Softmax ($\lambda=10$) & \textbf{73.21} & \textbf{92.57$^\circ$} & 88.49 & \textbf{96.25$^\circ$} & \textbf{65.91} & \textbf{93.84$^\circ$} & \textbf{86.96} & \textbf{96.09$^\circ$}\\ 
        LM-Softmax ($\lambda=20$) & \textbf{73.20} & \textbf{91.95$^\circ$} & \textbf{89.12} & \textbf{95.73$^\circ$} & \textbf{65.39} & \textbf{93.23$^\circ$} & \textbf{86.95} & \textbf{96.03$^\circ$}\\ 
         \bottomrule
    \end{tabular}
\end{table}


==> tables/imb_cifar100.tex <==
% \begin{table}[htbp]
% \scriptsize
%     \caption{Test accuracies and class margins on imbalanced CIFAR-100. The results with positive gains are \textbf{highlighted} (where * denotes learning with the regularization term in Eq. \ref{reg}).}
%     \centering
%     \begin{tabular}{l|cc|cc|cc|cc}
%         \toprule
%          Imbalance Type &  \multicolumn{4}{c|}{long-tailed} & \multicolumn{4}{c}{step}\\
%          \midrule
%          Imbalance Ratio &  \multicolumn{2}{c|}{100} & \multicolumn{2}{c|}{10} & \multicolumn{2}{c|}{100} & \multicolumn{2}{c}{10}\\
%          \midrule
%          Metric & ${acc}$ & $m_{cls}$ & $acc$ & $m_{cls}$ & $acc$ & $m_{cls}$ & $acc$ & $m_{cls}$\\
%          \midrule
%          CE & 32.99 & 71.47$^\circ$ & 57.06 & 74.21$^\circ$ & 41.18 & 65.65$^\circ$ & 54.79 & 70.57$^\circ$\\
%          Focal & 34.70 & 62.20$^\circ$ & 58.09 & 62.68$^\circ$ & 41.52 & 54.98$^\circ$ & 57.03 & 58.29$^\circ$\\
%          \midrule
%          LDAM & 44.01 & 9.437$^\circ$ & 62.54 & 83.02$^\circ$ & 42.09 & 0.1327$^\circ$ & 59.44 & 1.199$^\circ$\\
%          \textbf{LDAM*} & \textbf{44.76} & \textbf{51.54$^\circ$} & \textbf{63.17} & \textbf{87.61$^\circ$} & \textbf{44.78} & \textbf{32.51$^\circ$} & \textbf{61.11} & \textbf{86.74$^\circ$}\\
%          \midrule
%          CosFace & 38.36 & 13.88$^\circ$ & 60.94 & 81.52$^\circ$ & 39.94 & 0.1342$^\circ$ & 53.93 & 4.016$^\circ$\\
%          \textbf{CosFace*} & \textbf{41.87} & \textbf{70.20$^\circ$} & \textbf{61.18} & \textbf{85.99$^\circ$} & \textbf{42.25} & \textbf{40.48$^\circ$} & \textbf{59.24} & \textbf{87.45$^\circ$}\\
%          \midrule
%          ArcFace & 42.67 & 23.27$^\circ$ & 62.51 & 83.01$^\circ$ &42.45 & 0.6450$^\circ$ & 59.61 & 0.6537$^\circ$\\
%          \textbf{ArcFace*} & \textbf{43.91} & \textbf{65.52$^\circ$} & \textbf{62.65} & \textbf{84.22$^\circ$} & \textbf{44.68} & \textbf{34.58$^\circ$} & \textbf{59.92} & \textbf{79.18$^\circ$}\\
%          \midrule
%          NormFace & 42.82 & 34.23$^\circ$ & 62.78 & 81.95$^\circ$ & 42.40 & 0.1251$^\circ$ & 59.66 & 68.42$^\circ$\\
%          \textbf{NormFace*} & \textbf{44.04} & \textbf{77.23$^\circ$} & 62.55 & \textbf{84.73$^\circ$} & \textbf{44.36} & \textbf{43.98$^\circ$} & \textbf{61.10} & \textbf{80.79$^\circ$}\\
%          \midrule
%          LM-Softmax & 42.15 & 3.362$^\circ$ & 62.23 & 78.22$^\circ$ & 41.03 & 0.1371$^\circ$ & 56.45 & 0.1938$^\circ$\\
%          \textbf{LM-Softmax*} & \textbf{44.47} & \textbf{73.38$^\circ$} & \textbf{62.60} & \textbf{85.70$^\circ$} & \textbf{45.40} & \textbf{24.86$^\circ$} & \textbf{60.52} & \textbf{86.56$^\circ$}\\
%          \bottomrule
%     \end{tabular}
%     \label{im-cifar100}
% \end{table}

\begin{table}[htbp]
    \caption{Test accuracies and class margins on imbalanced CIFAR-100. The results with}
    \label{im-cifar100}
    \centering
    \begin{tabular}{l|cc|cc|cc|cc}
        \toprule
         Imbalance Type &  \multicolumn{4}{c|}{long-tailed} & \multicolumn{4}{c}{step}\\
         \midrule
         Imbalance Ratio &  \multicolumn{2}{c|}{100} & \multicolumn{2}{c|}{10} & \multicolumn{2}{c|}{100} & \multicolumn{2}{c}{10}\\
         \midrule
         Metric & acc & cls\_ m & acc & cls\_ m & acc & cls\_ m & acc & cls\_ m\\
         \midrule
         CE & 40.38 & 64.73$^\circ$ & 60.42 & 66.24$^\circ$ & 42.36 & 60.32$^\circ$ & 56.88 & 62.83$^\circ$\\
         Focal & 38.04 & 54.67$^\circ$ & 60.09 & 59.30$^\circ$ & 41.90 & 55.98$^\circ$ & 57.84 & 55.72$^\circ$\\
         \midrule
        CosFace ($\lambda=0$) & 34.91 & 4.73$^\circ$ & 60.60 & 70.82$^\circ$ & 40.36 & 0.76$^\circ$ & 47.56 & 8.56$^\circ$\\ 
        CosFace ($\lambda=1$) & \textbf{40.53} & \textbf{65.42$^\circ$} & 60.37 & \textbf{84.84$^\circ$} & \textbf{40.90} & \textbf{42.85$^\circ$} & \textbf{56.50} & \textbf{74.41$^\circ$}\\ 
        CosFace ($\lambda=2$) & \textbf{40.53} & \textbf{65.13$^\circ$} & \textbf{60.77} & \textbf{84.97$^\circ$} & \textbf{40.84} & \textbf{42.96$^\circ$} & \textbf{56.73} & \textbf{71.08$^\circ$}\\ 
        CosFace ($\lambda=5$) & \textbf{40.58} & \textbf{55.27$^\circ$} & 60.34 & \textbf{84.47$^\circ$} & \textbf{41.12} & \textbf{43.79$^\circ$} & \textbf{57.22} & \textbf{75.42$^\circ$}\\ 
        CosFace ($\lambda=10$) & \textbf{40.98} & \textbf{80.93$^\circ$} & 59.15 & \textbf{85.07$^\circ$} & \textbf{40.97} & \textbf{34.65$^\circ$} & \textbf{56.97} & \textbf{84.09$^\circ$}\\ 
        CosFace ($\lambda=20$) & \textbf{39.92} & \textbf{80.30$^\circ$} & 59.66 & \textbf{83.46$^\circ$} & \textbf{41.17} & \textbf{41.59$^\circ$} & \textbf{57.97} & \textbf{83.93$^\circ$}\\ 
        \midrule
        ArcFace ($\lambda=0$) & 42.77 & 13.22$^\circ$ & 63.21 & 67.73$^\circ$ & 41.47 & 0.50$^\circ$ & 58.89 & 0.37$^\circ$\\ 
        ArcFace ($\lambda=1$) & \textbf{43.97} & \textbf{52.75$^\circ$} & \textbf{63.67} & \textbf{71.52$^\circ$} & \textbf{44.45} & \textbf{0.71$^\circ$} & \textbf{61.11} & \textbf{62.38$^\circ$}\\ 
        ArcFace ($\lambda=2$) & \textbf{44.19} & \textbf{55.95$^\circ$} & \textbf{63.54} & \textbf{72.68$^\circ$} & \textbf{44.41} & \textbf{0.81$^\circ$} & \textbf{60.71} & \textbf{0.62$^\circ$}\\ 
        ArcFace ($\lambda=5$) & \textbf{44.68} & \textbf{56.60$^\circ$} & \textbf{63.80} & \textbf{73.45$^\circ$} & \textbf{43.79} & \textbf{0.61$^\circ$} & \textbf{60.30} & \textbf{63.68$^\circ$}\\ 
        ArcFace ($\lambda=10$) & \textbf{43.89} & \textbf{75.58$^\circ$} & \textbf{63.55} & \textbf{82.11$^\circ$} & \textbf{44.11} & \textbf{31.54$^\circ$} & \textbf{60.44} & \textbf{69.63$^\circ$}\\ 
        ArcFace ($\lambda=20$) & \textbf{43.55} & \textbf{75.28$^\circ$} & 62.10 & \textbf{81.00$^\circ$} & \textbf{44.26} & \textbf{32.10$^\circ$} & \textbf{60.79} & \textbf{79.85$^\circ$}\\ 
        \midrule
        NormFace ($\lambda=0$) & 43.71 & 16.11$^\circ$ & 63.50 & 71.26$^\circ$ & 41.93 & 1.36$^\circ$ & 59.85 & 21.32$^\circ$\\ 
        NormFace ($\lambda=1$) & \textbf{44.18} & \textbf{59.42$^\circ$} & \textbf{63.81} & \textbf{79.85$^\circ$} & \textbf{43.77} & \textbf{41.25$^\circ$} & \textbf{61.04} & \textbf{64.55$^\circ$}\\ 
        NormFace ($\lambda=2$) & \textbf{44.20} & \textbf{60.39$^\circ$} & \textbf{63.90} & \textbf{77.69$^\circ$} & \textbf{44.51} & \textbf{36.30$^\circ$} & \textbf{60.49} & \textbf{71.70$^\circ$}\\ 
        NormFace ($\lambda=5$) & \textbf{44.25} & \textbf{64.85$^\circ$} & \textbf{63.60} & \textbf{77.74$^\circ$} & \textbf{44.14} & \textbf{36.62$^\circ$} & \textbf{60.30} & \textbf{73.08$^\circ$}\\ 
        NormFace ($\lambda=10$) & 43.71 & \textbf{74.87$^\circ$} & 63.17 & \textbf{82.71$^\circ$} & \textbf{43.61} & \textbf{36.47$^\circ$} & \textbf{60.22} & \textbf{80.83$^\circ$}\\ 
        NormFace ($\lambda=20$) & 43.67 & \textbf{75.71$^\circ$} & 62.66 & \textbf{82.18$^\circ$} & \textbf{43.70} & \textbf{28.94$^\circ$} & \textbf{60.16} & \textbf{81.66$^\circ$}\\ 
        \midrule
        LDAM ($\lambda=0$) & 43.28 & 7.73$^\circ$ & 63.62 & 73.19$^\circ$ & 41.65 & 0.85$^\circ$ & 58.32 & 6.08$^\circ$\\ 
        LDAM ($\lambda=1$) & \textbf{44.18} & \textbf{71.00$^\circ$} & \textbf{63.95} & \textbf{84.49$^\circ$} & \textbf{44.14} & \textbf{39.14$^\circ$} & \textbf{60.52} & \textbf{71.43$^\circ$}\\ 
        LDAM ($\lambda=2$) & \textbf{44.90} & \textbf{67.95$^\circ$} & \textbf{64.12} & \textbf{85.81$^\circ$} & \textbf{44.40} & \textbf{36.96$^\circ$} & \textbf{60.83} & \textbf{75.22$^\circ$}\\ 
        LDAM ($\lambda=5$) & \textbf{45.23} & \textbf{70.96$^\circ$} & \textbf{64.18} & \textbf{85.03$^\circ$} & \textbf{43.80} & \textbf{40.03$^\circ$} & \textbf{60.83} & \textbf{72.27$^\circ$}\\ 
        LDAM ($\lambda=10$) & \textbf{43.53} & \textbf{81.42$^\circ$} & 63.05 & \textbf{85.62$^\circ$} & \textbf{44.48} & \textbf{43.26$^\circ$} & \textbf{60.39} & \textbf{83.06$^\circ$}\\ 
        LDAM ($\lambda=20$) & \textbf{43.85} & \textbf{79.65$^\circ$} & 62.64 & \textbf{84.87$^\circ$} & \textbf{44.17} & \textbf{37.66$^\circ$} & \textbf{60.28} & \textbf{84.31$^\circ$}\\ 
        \midrule
        LM-Softmax ($\lambda=0$) & 41.52 & 4.50$^\circ$ & 63.26 & 68.31$^\circ$ & 41.53 & 0.47$^\circ$ & 55.44 & 1.37$^\circ$\\ 
        LM-Softmax ($\lambda=1$) & \textbf{45.22} & \textbf{68.02$^\circ$} & \textbf{63.77} & \textbf{81.99$^\circ$} & \textbf{45.40} & \textbf{39.87$^\circ$} & \textbf{60.57} & \textbf{73.19$^\circ$}\\ 
        LM-Softmax ($\lambda=2$) & \textbf{44.90} & \textbf{67.90$^\circ$} & \textbf{63.39} & \textbf{82.93$^\circ$} & \textbf{45.17} & \textbf{38.29$^\circ$} & \textbf{60.73} & \textbf{74.78$^\circ$}\\ 
        LM-Softmax ($\lambda=5$) & \textbf{45.28} & \textbf{69.53$^\circ$} & \textbf{63.60} & \textbf{83.32$^\circ$} & \textbf{46.23} & \textbf{43.15$^\circ$} & \textbf{60.22} & \textbf{74.37$^\circ$}\\ 
        LM-Softmax ($\lambda=10$) & \textbf{44.13} & \textbf{78.90$^\circ$} & 62.89 & \textbf{85.39$^\circ$} & \textbf{45.06} & \textbf{46.69$^\circ$} & \textbf{60.48} & \textbf{7.94$^\circ$}\\ 
        LM-Softmax ($\lambda=20$) & \textbf{44.22} & \textbf{80.53$^\circ$} & \textbf{63.40} & \textbf{83.80$^\circ$} & \textbf{45.97} & \textbf{64.84$^\circ$} & \textbf{60.23} & \textbf{76.77$^\circ$}\\ 
         \bottomrule
    \end{tabular}
\end{table}
